Hermes: a Fast, Fault-Tolerant and Linearizable Replication Protocol

Today's datacenter applications are underpinned by datastores that are responsible for providing availability, consistency, and performance. For high availability in the presence of failures, these datastores replicate data across several nodes. This is accomplished with the help of a reliable replication protocol that is responsible for maintaining the replicas strongly-consistent even when faults occur. Strong consistency is preferred to weaker consistency models that cannot guarantee an intuitive behavior for the clients. Furthermore, to accommodate high demand at real-time latencies, datastores must deliver high throughput and low latency. This work introduces Hermes, a broadcast-based reliable replication protocol for in-memory datastores that provides both high throughput and low latency by enabling local reads and fully-concurrent fast writes at all replicas. Hermes couples logical timestamps with cache-coherence-inspired invalidations to guarantee linearizability, avoid write serialization at a centralized ordering point, resolve write conflicts locally at each replica (hence ensuring that writes never abort) and provide fault-tolerance via replayable writes. Our implementation of Hermes over an RDMA-enabled reliable datastore with five replicas shows that Hermes consistently achieves higher throughput than state-of-the-art RDMA-based reliable protocols (ZAB and CRAQ) across all write ratios while also significantly reducing tail latency. At 5% writes, the tail latency of Hermes is 3.6X lower than that of CRAQ and ZAB.

==> 4_incl_graphics/eval-derecho.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Graphs/derecho_comparison.pdf} 
  \vspace{-2.5em}
  \caption{Write-only throughput of Derecho and HermesKV single thread, while varying object size. [Uniform traffic, 5 nodes]}
  \vspace{-1.5em}
  \label{fig:derecho}
\end{figure}

==> 4_incl_graphics/eval-failures.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Graphs/xPut_with_failure_write_rate_5_line_plot.pdf} 
  \vspace{-2.5em}
  \caption{Throughput of HermesKV when injecting a failure. [Uniform traffic, 5 nodes, timeout=150ms]}
  \vspace{-1.5em}
  \label{fig:failure-throughput}
\end{figure}

==> 4_incl_graphics/eval-latency.tex <==

\begin{figure*}[t]
%%%%%%% Uniform Figure %%%%%%%%%
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{Graphs/write_rate_latency_study_uniform_out.pdf}
  \captionsetup{font=Big, width=0.85\linewidth}
  \vspace{-0.25em}
  \caption{Uniform}
  \label{fig:latency-uni}
  \end{subfigure}%
%%%%%%% Skew Figure %%%%%%%%%
  \begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{Graphs/write_rate_latency_study_skew_out.pdf}
  \captionsetup{font=big, width=0.85\linewidth}
  \vspace{-0.25em}
  \caption{Skewed [Zipfian exponent 0.99]}
  \label{fig:latency-skew}
  \end{subfigure}
  \vspace{-1.25em}
  \caption{Median and 99th\% latency while varying the write rate. [5 nodes]}
  \vspace{-1.5em}
\end{figure*}

==> 4_incl_graphics/eval-latency_xput.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Graphs/latency_vs_xPut_all_write_rate_5_line_plot.pdf} 
  \vspace{-2em}
  \caption{Latency vs Throughput. [Uniform traffic, 5\% write ratio, 5 nodes]}
  \label{fig:latency}
  \vspace{-1.25em}
\end{figure}

==> 4_incl_graphics/eval-scalability.tex <==
\begin{figure}[t]
%   \centering
  \includegraphics[width=0.5\textwidth]{Graphs/sclability_study_varying_write_rate_1_and_20_double_column.pdf} 
  \vspace{-2em}
  \caption{Scalability study. [Uniform traffic] }
  \vspace{-1.5em}
  \label{fig:scalability-line}
\end{figure}

==> 4_incl_graphics/eval-table.tex <==
\vspace{-80pt}
\begin{adjustbox}{max width=0.30\textwidth}

\begin{tikzpicture}
\centering
\node (table) [inner sep=-0pt] {
\begin{tabular}{l|l|l|l|l|c}
\rowcolor[HTML]{9B9B9B} 
\cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{local reads}} & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{writes}} \\ \cline{2-6} 
\rowcolor[HTML]{9B9B9B} 
\multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{systems}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Con.} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}DC} \\
\textbf{HermesKV} & single RM & Lin & inter-key & 1 RTT & \cmark \\
\textbf{rCRAQ} & single RM & Lin & inter-key & O(\textit{n}) & \xmark \\
\textbf{rZAB} & no need & SC & serializes all & 1.5 RTT & \xmark \\
\textbf{Derecho} & no need & SC & lock-step apply & 1.5 RTT & \cmark
\end{tabular}

};
\draw [rounded corners=.3em] (table.north west) rectangle (table.south east);

\end{tikzpicture}

\end{adjustbox}

\caption{
Leases and consistency (Con.) for local reads and write features of evaluated systems. 
% Write concurrency and local reads lease usage and consistency for evaluated systems.
SC is sequentially consistent, DC is decentralized, \textit{n} is number of replicas.
}
\label{tab:eval}
\vspace{-20pt}

==> 4_incl_graphics/eval-write_only.tex <==
\begin{figure}[t]
%   \centering
%   \includegraphics[width=0.5\textwidth]{Graphs/systems_comparison.pdf} 
  \input{Miscellaneous/Eval-write-only.tex}
  \vspace{-1em}
  \caption{Write-only study. [Uniform traffic, 5 nodes] }
  \vspace{-1.5em}
  \label{fig:write-only}
\end{figure}

==> 4_incl_graphics/eval-xput-n-table.tex <==
\begin{figure*}[t]
  \begin{subfigure}[b]{0.20\textwidth}
  
    \begin{adjustbox}{max width=0.99\textwidth}

    \begin{tikzpicture}
    \node (table) [inner sep=-0pt] {
    \begin{tabular}{l|l|l|l|l|c}
    \rowcolor[HTML]{9B9B9B} 
    \cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{local reads}} & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{writes}} \\ \cline{2-6} 
    \rowcolor[HTML]{9B9B9B} 
    \multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{systems}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Con.} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}DC} \\
    \textbf{HermesKV} & single RM & Lin & inter-key & 1 RTT & \cmark \\
    \textbf{rCRAQ} & single RM & Lin & inter-key & O(\textit{n}) & \xmark \\
    \textbf{rZAB} & no need & SC & serializes all & 1.5 RTT & \xmark \\
    \textbf{Derecho} & no need & SC & lock-step apply & 1.5 RTT & \cmark
    \end{tabular}
    };
    \draw [rounded corners=.3em] (table.north west) rectangle (table.south east);
    % \caption{Leases and consistency (Con.) for local reads and write features of evaluated systems. 
    % % Write concurrency and local reads lease usage and consistency for evaluated systems.
    % SC is sequentially consistent, DC is decentralized, \textit{n} is number of replicas.}
    % \label{tab:eval}
    \end{tikzpicture}
    \end{adjustbox}
    % \captionsetup{width=0.85\linewidth}
    \vspace{-0.25em}
    

  \end{subfigure}
  
  %
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
    \vspace{-0.9em}
    \caption{Uniform}
    \label{fig:write-rate}
    % \includegraphics[width=\textwidth]{2_graphs/write_rate_latency_study_uniform_out.pdf}
    % \captionsetup{width=0.85\linewidth}
    % \vspace{-1.8em}
    % \caption{Median and 99th\% [Uniform traffic]}
    % \label{fig:latency-uni}
  \end{subfigure}
  %
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{2_graphs/skew_99_and_write_rate_performance_study.pdf}
    \vspace{-0.9em}
    \caption{Skewed [Zipfian exponent 0.99]}
    \label{fig:skew-line}
    % \includegraphics[width=\textwidth]{2_graphs/write_rate_latency_study_skew_out.pdf}
    % \captionsetup{width=0.85\linewidth}
    % \vspace{-1.8em}
    % \caption{Median and 99th\% [Zipfian 0.99]}
    % \label{fig:latency-skew}
  \end{subfigure}
    \vspace{-0.75em}
  \caption{Throughput for $1\%$ to $100\%$ write ratio. [5 nodes]}
  \vspace{-15pt}
%   \vspace{-2.5em}
%   \caption{Latency analysis. [5 nodes] }
%   \vspace{-10pt}
\end{figure*}


% \begin{figure*}[t]
% \captionsetup[figure]{labelfont={bf},name={Fig.},labelsep=period}
% \captionsetup[subfigure]{labelfont={bf},name={Fig.},labelsep=period}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% %%%%%%% Uniform Figure %%%%%%%%%
% %   \hspace{30pt}
%   \begin{subfigure}{0.32\textwidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
%   \vspace{-0.9em}
%   \caption{Uniform}
%   \label{fig:write-rate}
%   \end{subfigure}%
% %%%%%%% Skew Figure %%%%%%%%%
% % \hspace{100pt}
%   \begin{subfigure}{0.32\textwidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{2_graphs/skew_99_and_write_rate_performance_study.pdf}
%   \vspace{-0.9em}
%   \caption{Skewed [Zipfian exponent 0.99]}
%   \label{fig:skew-line}
%   \end{subfigure}
%   \vspace{-0.75em}
%   \caption{Throughput for $1\%$ to $100\%$ write ratio. [5 nodes]}
%   \vspace{-15pt}
% \end{figure*}

\begin{figure*}[t]
\setkeys{Gin}{width=1.05\linewidth}
\begin{tabularx}{\linewidth}{XXX}
    \begin{adjustbox}{max width=0.33\textwidth}
    \begin{tikzpicture}
    \node (table) [inner sep=-0pt] {
    \begin{tabular}{l|l|l|l|l|c}
    \rowcolor[HTML]{9B9B9B} 
    \cellcolor[HTML]{9B9B9B} & \multicolumn{2}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{local reads}} & \multicolumn{3}{c|}{\cellcolor[HTML]{9B9B9B}\textbf{writes}} \\ \cline{2-6} 
    \rowcolor[HTML]{9B9B9B} 
    \multirow{-2}{*}{\cellcolor[HTML]{9B9B9B}\textbf{systems}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Leases} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Con.} & \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}Concurrency} & Latency & \multicolumn{1}{l}{\cellcolor[HTML]{9B9B9B}DC} \\
    \textbf{HermesKV} & single RM & Lin & inter-key & 1 RTT & \cmark \\
    \textbf{rCRAQ} & single RM & Lin & inter-key & O(\textit{n}) & \xmark \\
    \textbf{rZAB} & no need & SC & serializes all & 1.5 RTT & \xmark \\
    \textbf{Derecho} & no need & SC & lock-step apply & 1.5 RTT & \cmark
    \end{tabular}
    };
    \draw [rounded corners=.3em] (table.north west) rectangle (table.south east);
   
    \end{tikzpicture}
    \end{adjustbox}
     \caption{Leases and consistency (Con.) for local reads and write features of evaluated systems. 
    % Write concurrency and local reads lease usage and consistency for evaluated systems.
    SC is sequentially consistent, DC is decentralized, \textit{n} is number of replicas.}
    \label{tab:eval}
&
    \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
    \vspace{-0.9em}
    \caption{Uniform}
    \label{fig:write-rate}
&
    \includegraphics[width=0.9\linewidth]{2_graphs/skew_99_and_write_rate_performance_study.pdf}
    \vspace{-0.9em}
    \caption{Skewed [Zipfian exponent 0.99]}
    \label{fig:skew-line}
\end{tabularx}
\vspace{-20pt}
\end{figure*}

==> 4_incl_graphics/eval-xput-triple.tex <==

% \begin{figure*}[t]
% \captionsetup[figure]{labelfont={bf},name={Fig.},labelsep=period}
% \captionsetup[subfigure]{labelfont={bf},name={Fig.},labelsep=period}


% \begin{figure*}[t]
% \setkeys{Gin}{width=1.05\linewidth}
% \begin{tabularx}{\linewidth}{XXX}
%     % \begin{adjustbox}{max width=0.33\textwidth}
    
%     \input{4_incl_graphics/eval-table.tex}
%     % \includegraphics[width=0.9\linewidth]{eval-table}
    
    
%     % \input{3_misc/Evaluation-Table.tex}
%     % \begin{figure}[t]
%     % \begin{subfigure}[b]{0.32\textwidth}
%     % \centering
%     % \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
%     % \vspace{-0.9em}
%     % \caption{Uniform}
%     % \label{fig:write-rate}
%     % \end{subfigure}
%     % \end{figure}
% &
% %  \begin{figure}[t]
% %   \begin{subfigure}[b]{0.32\textwidth}
%     % \centering
%     \includegraphics[width=0.9\linewidth]{2_graphs/write_rate_performance_study.pdf}
%     \vspace{-0.9em}
%     \subcaption{Uniform}
%     \label{fig:write-rate}
% %   \end{subfigure}
% %   \end{figure}
%   %
%   &
% %   \begin{figure}[t]
% %   \begin{subfigure}[b]{0.32\textwidth}
%     % \centering
%     \includegraphics[width=0.9\linewidth]{2_graphs/skew_99_and_write_rate_performance_study.pdf}
%     \vspace{-0.9em}
%     \subcaption{Skewed [Zipfian exponent 0.99]}
%     \label{fig:skew-line}
% %   \end{subfigure}
%     \vspace{-0.75em}
% %   \end{figure}
%  \end{tabularx}
% \vspace{-40pt}
% \hspace{150pt} \caption{Throughput for $1\%$ to $100\%$ write ratio. [5 nodes]}
% \vspace{-15pt}
% \end{figure*}


\begin{figure*}[t]
\setkeys{Gin}{width=1.05\linewidth}
\begin{tabularx}{\linewidth}{XXX}
    % \begin{adjustbox}{max width=0.33\textwidth}
    
    \input{3_misc/Evaluation-Table.tex}
    % \input{4_incl_graphics/eval-table.tex}
    
&
    \input{4_incl_graphics/eval-xput.tex}
% 
%   \end{figure}
 \end{tabularx}
% \vspace{-40pt}
% \hspace{150pt} \caption{Throughput for $1\%$ to $100\%$ write ratio. [5 nodes]}
% \vspace{-15pt}
\end{figure*}

==> Makefile <==
#
## Makefile for acmart package
#

PACKAGE=acmart

MAIN_TEX=HermesAsplos20


TEXSRCS := $(wildcard *.tex) \
	   $(wildcard ./0_sections/*.tex) \
	   $(wildcard ./3_misc/*.tex) \
	   $(wildcard ./4_incl_graphics/*.tex)


all:  $(MAIN_TEX).pdf

%.cls:   %.ins %.dtx  
		pdflatex $<

$(MAIN_TEX).pdf:  $(PACKAGE).cls ACM-Reference-Format.bst $(TEXSRCS)
		pdflatex $(MAIN_TEX)
		- bibtex $(MAIN_TEX)
		pdflatex $(MAIN_TEX)
		pdflatex $(MAIN_TEX)

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

pdf-clean: clean
	$(RM) $(MAIN_TEX).pdf

